SignLLM: Sign Language Production Large Language Models

In this paper, we propose SignLLM, a multilingual Sign Language Production (SLP) large language model, which includes two novel multilingual SLP modes MLSF and Prompt2LangGloss that allow sign language gestures generation from query texts input and question-style prompts input respectively. Both modes can use a new RL loss based on reinforcement learning and a new RL module named Priority Learning Channel. These RL components can accelerate the training by enhancing the model's capability to sample high-quality data. To train SignLLM, we introduce Prompt2Sign, a comprehensive multilingual sign language dataset, which builds from public data, including American Sign Language (ASL) and seven others. This dataset standardizes information by extracting pose information from sign language videos into a unified compressed format. We extensively evaluate SignLLM, demonstrating that our model achieves state-of-the-art performance on SLP tasks across eight sign languages.

==> sec/optional_subsec/ext_vis.tex <==
\begin{figure}[ht]
    \centering
    \footnotesize
    \includegraphics[width=\linewidth]{fig/expand.drawio.png}
    \vspace{-18pt}
    \caption{\textbf{Extensibility Presentation:} We used five motion capture models and five sign language rendering models to represent the final effect of production.}
    \vspace{-14pt}
    \label{fig:expand}
\end{figure}

\input{table/visual}

\vspace{-12pt}
\paragraph{Extensibility \& Visual Presentation.}

In Figure \ref{fig:expand}, the upper half of it is obtained either directly or indirectly by reading our \ourLLMmethodName{} output sequence through motion capture \cite{chen2023executing,cai2023smplerx,smpl} software or models (The official website for more software is in the supplementary materials), while the lower half of the image comes from the commonly used Pose2Vid \cite{mallya2020world,tulyakov2018mocogan,vondrick2016generating,Rombach_2022_CVPR,zhang2023adding,hu2021lora} or Pose2Img \cite{isola2017image,radford2015unsupervised,wang2018high,zhu2017unpaired} models in sign language. We explored the influence of different forms on performance as shown in Table \ref{tab:visual}, and found that in the field of sign language, the motion capture software was superior to the visual model in most cases, because there was less loss and no stroboscopic problems, and even exceeded the visual model to more than 24 frames per second. 
%the motion capture was better than the visual methods, and future researchers could explore in this direction.
%We also conducted more qualitative assessments of the images, which were stored in the .
%and appendix \ref{paragraph:more_Visual_Study}

==> sec/optional_subsec/first_intro_long.tex <==
% Sign Intro
\acf{slp} aims to synthesize human-like sign avatars from text inputs.
Deep learning-based SLP approaches \cite{saunders2020progressive,saunders2021continuous,huang2021towards,saunders2021mixed,saunders2021skeletal} typically involve sequential steps from text to gloss (\ie, a type of textual vocabulary representing gestures or postures), gloss to pose \cite{carreira-2017-i3d,MediaPipe},
%skeletal pose \cite{cao2018openpose}, dense pose \cite{qiu2021dense,huang2017densely,Zhao-arxiv-2022-Dense}, or other formats \cite{smpl,carreira-2017-i3d,MediaPipe}. 
and finally rendering pose videos into more engaging human-like avatar videos. These processes are complex and challenging to simplify, making sign language data acquisition and processing difficult. This challenge has significantly dampened researchers' enthusiasm and progress over a considerable period, with the majority of studies in the past decade relying on a German sign language (GSL) dataset named PHOENIX14T \cite{forster2012rwth, koller15:cslr} and other lesser-known languages datasets \cite{Duarte_2021_how2sign,RWTH-PHOENIX-Weather-2014,muller-etal-2023-findings,Ronchetti2016,Ham21,9210578} for \textbf{S}ign \textbf{L}anguage \textbf{P}roduction, \textbf{R}ecognition, and \textbf{T}ranslation tasks (SLP, SLR and SLT). Additionally, the use of various tools adhering to different standards \cite{7298594,guler2018densepose,smpl} by different researchers further complicates the task. Recent work \cite{slt-how2sign-wicv2023,fang2024signdiffdiffusionmodelsamerican,Bohacek_2022_WACV} based on the American sign language (ASL) dataset \cite{duarte2021how2sign,shi-etal-2022-openASL} is almost nascent, and the research progress on other minority languages is also very limited \cite{ebling2016automatic,8778347}.
%SLR \cite{camgoz2020sign,Bohacek_2022_WACV,slt-how2sign-wicv2023}, SLP \cite{saunders2021continuous,saunders2020progressive,zelinka2020neural,huang2021towards,brentari2018production}, human-like image production \cite{stoll2018sign,zelinka2020neural,saunders2020adversarial}, and long-video SLT \cite{camgoz2020sign,slt-how2sign-wicv2023} tasks.
%The duration and vocabulary of How2Sign are approximately 7.53 and 5.74 times larger than the commonly used PHOENIX14T, respectively.
%RWTH-PHOENIX-Weather-2014T

==> sec/optional_subsec/method_motivation.tex <==
\subsection{Motivation} \label{sec:Motivation}

For multilingual sign language production and large language models, the challenges lie in the convenient switching or expansion of the types of sign language, and the availability of a sufficiently large amount of high-quality data. Accordingly, we propose a new MLSF framework to handle the case of shared parameters among various sign languages. We incorporate two new components, "Text2LangGloss" and "Priority Learning Channel", to separately address the issues of multiple sign languages using a set of parameters (based on learning from prompt words) and overfitting as well as prolonged training time with large-scale data. We have a reinforcement learning-based loss adapted to the new model, which expands the possibilities of sign language production.

==> sec/optional_subsec/method_prompt2pose.tex <==
\vspace{-8pt}
\paragraph{Prompt2Text \& Text2Pose} \label{paragraph:prompt_to_pose}

The first part of our new method is the conversion of a given prompt into spoken language text, essentially mirroring the previously described operation "Text to Gloss" (Section \ref{paragraph:text_to_pose}). The principal distinction between these two lies in the translation target: whilst "Text to Gloss" aims to generate a gloss sequence as output, the goal of "Prompt to Text" is to generate textual sequences corresponding to the spoken language.

The Encoder-Decoder transformer framework is utilised in this stage similar to its "Text to Gloss" equivalent, with the transformation defined as follows:
\begin{equation}
    f_{t} = E_{Prompt2Text}(v_{t} | v_{1:\mathcal{T}})
\end{equation}
\vspace{-12pt}
\begin{equation}
    text_{w+1} = D_{Prompt2Text}(text_{w}  | text_{1:w-1} , f_{1:\mathcal{T}})
\end{equation}
Here, $f_{t}$ represents the encoded source token, and $text_{w}$ represents the text at timestep $w$, which is the target token. The pose at each timestep is calculated as $\hat{y}_{w} = \operatorname*{argmax}_{i} (text_{w})$ until a specific termination condition is met.
Our new "Text to Pose" operates likewise through the original "Gloss to Pose" channel, hence further elaboration is unwarranted. The visual representation, shown in the middle of Figure \ref{fig:text2langloss}, shows the Prompt2Text channel with a tagger enhancement trick.

==> sec/optional_subsec/related_work_RL.tex <==
\vspace{-8pt}
\paragraph{Reinforcement Learning}

in the training or fine-tuning of large models is a common strategy \cite{hermann-etal-2017-grounded, misra-etal-2017-mapping, bahdanau-etal-2018-learning, colas-etal-2020-language, chevalierboisvert-etal-2019-babyai}. 
At the heart of reinforcement learning (RL) is the concept of a Markov Decision Process (MDP), an extension of Markov chains. 
%At the heart of reinforcement learning is the concept of a Markov Decision Process (MDP), an extension of Markov chains, which involves a finite set of states, a finite set of actions, state transition probabilities, and a reward function.
The MDP delineates the interaction \cite{yuan-etal-2021-florence,devlin-etal-2019-bert,brown-etal-2020-language} between an intelligent agent and the environment, wherein the agent chooses actions based on various states, and the environment imposes rewards or penalties on the agent based on the action and the current state, leading to a transition to the next state.
An optimal policy is the mapping from state $s$ to action $a$ that maximizes the total expected return:
\begin{equation}
\pi^* = \arg\max_{\pi} \mathbb{E}[G_t | s_t =s, \pi]
\end{equation}
where $G_t = \sum_{k=0}^{\infty}\gamma^k R_{t+k+1}$, $0 \leq \gamma < 1$ is the discount factor, and $\mathbb{E}[]$ is the expectation operator.
Given that the \ac{slp} process aligns with the definition and can be reformed by the MDP, as an agent activity that follows language instructions \cite{luketina2019survey}, we simply simulate this concept to fine-tune our generation model. However, since the training scenario of sign language does not involve interacting with an environment that has another agent, more like a plain text interaction (i.e. performing textual commands given textual observations \cite{shridhar-etal-2021-alfword}), our RL strategy is not a typical one, but rather only partially applied to component modules.

%Our objective is to train a Sign Language Pose network to generate sequences of 3D skeleton poses on How2Sign. Initially, we extract 2D joint positions from each video using the OpenPose method \cite{cao2018openpose}. We then incorporate the skeletal model estimation improvements introduced in  Zelink \etal \cite{zelinka2020neural} to transform the 2D joint positions into their corresponding 3D counterparts and run on eight RTX4090 GPUs for ten days. Moreover, we employ an iterative inverse kinematics approach to minimize the 3D pose while preserving consistent bone lengths and correcting any misplaced joints. Finally, following a similar approach as proposed in Stoll \etal \cite{stoll2018sign}, we normalize the skeletal data and represent the 3D joints using Cartesian coordinates $x$, $y$, and $z$. Finally, we read the relevant data and delete the unqualified data such as NaN, 0, or replace it with the average median of the data. Finally, we condensed the data to about 1/5 of the original.

%The data required for the diffusion model/Vid2Vid model is processed according to the official documents, and the PHOENIX14T used for the preprocessing is shared by related open sources\footnote{https://github.com/BenSaunders27/ProgressiveTransformersSLP}. Our tens of scripts and thousands of lines of preprocessing tools are available in supplementary materials and will be open-sourced.

%We build our Text to Gloss models with 2 layers, 4 heads, and a hidden size of 128 and our \FrameSelectionNet{} with 2 layers, 4 heads, and 64 hidden sizes. We set the interpolation frames, $\mathcal{N}_{LI}$, to 5 and the learning rate to $10^{-3}$. Our code is based on JoeyNMT \cite{JoeyNMT}, and implemented using PyTorch \cite{paszke2017automatic}.

==> sec/optional_subsec/suppl_cover.tex <==
\twocolumn[{%
\renewcommand\twocolumn[1][]{#1}%
\maketitlesupplementary
\begin{center}
    \centering
    \includegraphics[width=.99\textwidth]{fig/cover_old.drawio.png}
    \captionof{figure}{\textbf{Bilingual Sign Language Production:} (a) Enter an American English or German sentence you want to translate; (b) Our \ourLLMmethodName{} then translates the text into a continuous skeleton pose sequence, and supports prompt word input; (c) The textual correspondence of sign language skeletal postures varies across different countries. These postures can be post-processed into more comprehensible images via conditional image generation models such as ControlNet.
    %Skeletal postures for sign language, which vary among different countries, can be subsequently processed by Conditional Control Image Generation Models like ControlNet.
    }
    \label{fig:cover_old}
\end{center}
}]

==> sec/optional_subsec/suppl_more_intro.tex <==
\section{More Introduction}

% Proposed method
In this paper, we introduce the first large-scale model for bilingual sign language production and construct the largest standardized bilingual sign language dataset to date. Initially, we propose a Multi-Language Switching Framework (MLSF) for \ac{slp}, based on state-of-the-art work in related fields. This framework dynamically incorporates an increasing number of encoders-decoders, enabling concurrent production of diverse sign languages. With two pipelines, text2gloss2pose and text2pose, it facilitates the production of a variety of sign language skeletal postures.

% MLSF part
In order to enable the MLSF framework to support static single-group coders and decoders for multilingual sign language production, we have developed two enhanced modules specifically improved for non-dynamic multilingual production and large-scale data training strategies. To avoid overfitting and redundant training caused by large datasets, we have for the first time introduced a novel loss based on the concept of reinforcement learning in sign language. This can reasonably prevent the problem of lengthy training times caused by large datasets, and also make it possible to seriously learn sign languages that are not known.

% Prompt2Sign part
In order to train \ourLLMmethodName{} with our new framework, we have constructed a new dataset named Prompt2Sign. It currently primarily sources from How2Sign and PHOENIX-14T, and we have spent several months recreating and optimizing them according to our model standards, reducing the space they occupy to one-tenth of their original size without any loss of data. To equip \ourLLMmethodName{} with conversational capabilities, we have synthesized 40,000 snippet prompts, making Prompt2Sign the most suitable dataset for large models of sign language. It can also rewrite prompts to enhance the robustness of large models, making it the largest dataset for future training of large sign language models.

==> sec/optional_subsec/suppl_more_method.tex <==
\section{More Details of Methodology}

\subsection{Motivation} \label{sec:Motivation}

For multilingual sign language production and large language models, the challenges lie in the convenient switching or expansion of the types of sign language, and the availability of a sufficiently large amount of high-quality data. Accordingly, we propose a new MLSF framework to handle the case of shared parameters among various sign languages. We incorporate two new components, "Text2LangGloss" and "Priority Learning Channel", to separately address the issues of multiple sign languages using a set of parameters (based on learning from prompt words) and overfitting as well as prolonged training time with large-scale data. We have a reinforcement learning-based loss adapted to the new model, which expands the possibilities of sign language production.

\subsection{Our innovative BSLP}

\paragraph{Multi-Language Switching Framework}

The profundity manifest in the presented piece of code lies in its capacity for dynamic language adaptation in the context of an encoder-decoder framework, specifically tailored for sign languages. Utilizing Python dictionaries, this paradigm ingeniously allows different encoders and decoders pertaining to distinct languages to be introduced into the model.

Given the set of encoders $\mathcal{E} = \{\epsilon_1, \epsilon_2, \ldots, \epsilon_n\}$ and decoders $\mathcal{D} = \{\delta_1, \delta_2, \ldots, \delta_n\}$ corresponding to $n$ languages, the novel implementation specifically assigns an encoder and decoder out of $\mathcal{E}$ and $\mathcal{D}$, respectively, determined by the language $\mathcal{L}$.
The ascription operation is formalized as $\text{Enc}_{\mathcal{L}} = \mathcal{E}_\mathcal{L}$ and $\text{Dec}_{\mathcal{L}} = \mathcal{D}_\mathcal{L}$, effectively setting the language-specific components for the current run.

The fortification of this framework provides an unequivocal advantage of incorporating a wide array of sign languages into the model, enhancing the flexibility and scalability, while also cutting down on extraneous computational cost typically associated with maintaining separate models for each language. Consequently, this dynamic substitution underscores the model's ability to be a universally applicable abstract sign language translation model.

The crowning achievement lies not only in the dexterity of the code but also in the mathematical robustness of the approach itself. In a sense, it placidly embeds a discrete 'choice' function $\chi: \mathcal{L} \to \mathcal{E} \times \mathcal{D}$ mapping languages to a tuple of encoder-decoder pairs, leveraging the power of modern functional programming paradigms alongside the inarguable efficacy of the foundational mathematical structures.
This gaping stride resonates well with the tenets of a cutting-edge approach to machine learning, focusing equally on the mathematical grants of versatility and the practical considerations of optimality and computational efficiency.

\paragraph{Text2LangGloss}

In the realm of sign language generation, Gloss plays a pivotal role. Acting as a textual depiction of sign language gestures, Gloss forms a crucial intermediary in a text-to-gloss (T2G) model. We propose an improvement to this model, which encompasses the attachment of an additional linguistic attribute to each Gloss during the parsing and tokenizing stages. For instance, a typical Gloss token "xxx" can be modified to "ASL\_xxx", which adds an element of conditional input to sign language generation.

The advantages of employing this method are manifold. Initially, it facilitates a single model to concurrently manage parameters for numerous languages, thereby nullifying the necessity for alternating between platforms or models. This alleviates a prominent intricacy associated with linguistics—overlapping of the semantic essence of words across different languages, which may lead to potential ambiguity. Our LangGloss as a conditional input helps to stratify these overlaps, subsequently significantly diminishing the chance of model errors.

Moreover, our approach augments the model robustness. In an instance where all Gloss tokens start with the prefix "ASL\_" and a single "GSL\_" token is inaccurately included, our refined model recognizes this token as an error given the pre-set conditions, thereby substantially mitigating the likelihood of errors, potentially by a factor of 10 or even 100. Therefore, our Text2LangGloss method introduces a strategic and streamlined solution for sign language generation across various languages.

Given a spoken language sequence, it is initially converted into a sequence of gloss tokens, each supplemented with its corresponding linguistic attribute, forming a LangGloss sequence. As such, a source sequence denoted by $\mathcal{X} = (x_{1},...,x_{\mathcal{T}})$ in the spoken language is mapped to a LangGloss sequence indicated by $\mathcal{Z} = (L_{1}z_{1},...,L_{\mathcal{W}}z_{\mathcal{W}})$, wherein $L_{i}$ refers to the linguistic attribute of each gloss token and $\mathcal{W}$ implies the total count of LangGloss tokens.

The equations are defined as follows:

\begin{equation}
\label{eq:T2LG_encoder}
    f_{t} = E_{T2LG}(x_{t} | x_{1:t-1})
\end{equation}

\begin{equation}
\label{eq:T2LG_decoder}
    g_{w+1} = D_{T2LG}(g_{w}  | g_{1:w} , f_{1:\mathcal{T}})
\end{equation}

Here, $f_{t}$ and $g_{w}$ denote the encoded source and target tokens respectively, with $g_{0}$ initialized as the encoding of the special $\mathrm{<bos>}$ token. The LangGloss tokens are allocated based on the maximum decoder output value, i.e., $ z_{w} = \operatorname*{argmax}_{i} (g_{w})$, a procedure that continues until the special $\mathrm{<eos>}$ token is predicted. 

Ultimately, this framework empowers the model to maintain parameters for various sign languages concurrently, minimizing any potential ambiguity during prediction and enhancing the robustness of the system.

\paragraph{Priority Learning Channel} 

The cornerstone of our methodology is the introduction of a Priority Learning Channel (PLC) that inherently directs the model's attention towards high-reward data samples. The principal hypothesis underwriting this approach is that such targeted learning would not only expeditiously aid in model convergence but would also boost the model's overall performance. 

We define the reward of each data sample as the absolute difference between the model's prediction and the actual target, mathematically denoted as $r(i) = \|y_i-\hat{y}_i\|$. These rewards are converted into sampling probabilities for each data sample according to 
\begin{equation}
 P(i) = \frac{ r(i)^\eta}{\sum_{j \in S} r(j)^\eta}, 
\end{equation}
where $\eta$ regulates the intensity of prioritization, and $S$ represents the dataset. By employing these sampling probabilities, the choice of data samples for each batch is no longer uniform but regulated by their respective rewards. 

The per-instance RL loss, $L(i)$, is computed for the chosen instances, which is then used to optimize the model parameters following the policy gradient theorem. This procedure is formally expressed as 
\begin{equation}
Minimize \; \; E_{i \sim P(i)}[L(i)]
\end{equation}
By continually updating the model based on the most rewarding examples, the PLC bridges the gap between reinforcement learning and supervised learning for sequence prediction tasks. The adaptive nature of the PLC ensures that the model's focus shifts in accordance with the model's evolving knowledge, thereby accelerating the learning process. 

This novel methodology heralds a shift from traditional modes of sequence learning and has the potential to bring about substantial improvements in the efficiency and effectiveness of such models.

\paragraph{Reinforcement Learning Loss}\label{paragraph:more_RL_Loss}

In the context of Reinforcement Learning (RL), we formulate the machine learning task into a Policy Learning problem. The goal of a typical RL agent, often formalized as a policy $\pi$, is to maximize the expected cumulative reward over a series of states $s_t$ and corresponding actions $a_t$:
\[
\pi^* = \underset{\pi}{\operatorname{argmax}} \, \mathbb{E}_{\pi}\left[\sum_{t=0}^{T} r_t\right]
\]
where $r_t$ is the reward at time $t$ and $T$ is the terminal time step. 

Now mapping this RL framework to our sequence learning context, the state $s_t$ can be seen as the input sequence, and the action $a_t$ exemplifies the output sequence, whilst the reward $r_t$ is a signal reflective of how good the predicted sequence is, measured against the target sequence. The better the correspondence between the prediction and the target, the higher the reward. One can argue, the reward can essentially be perceived as being inversely proportional to the Mean Squared Error loss that quantifies this discrepancy:
\[
r = -\frac{1}{N}\sum_{i=1}^{N}(y_i-\hat{y}_i)^2
\]
where $y_i$ is the target sequence, $\hat{y}_i$ is the predicted sequence, and $N$ is the count of the predictions.

This adopting of reinforcement learning parlance thereby innovativeley rephrases the conventional supervised learning problem of finding a set of optimal parameters $\theta$ which minimize the mean squared error loss into a setup geared towards maximizing the expected cumulative reward:

\begin{equation}
\begin{aligned}
\theta^* &= \underset{\theta}{\operatorname{argmax}} \, \mathbb{E}_{\theta}\left[\sum_{t=0}^{T} r_t\right] \\ &= \underset{\theta}{\operatorname{argmin}} \, \mathbb{E}_{\theta}\left[\sum_{t=0}^{T} L(y_t, M(x_t))\right]
\end{aligned}
\end{equation}

where $L$ denotes the MSE loss function, $M$ is the model and $x_t$, $y_t$ are the model inputs and corresponding targets respectively.

The optimal parameters are found by using gradient descent, where the parameters are updated proportionally to the gradient of the expected cumulative reward w.r.t model parameters:

\[
\theta_{t+1} = \theta_t - \alpha \nabla R
\]

where $R$ is the cumulative reward equivalent to $-\sum_{t=0}^{T} L(y_t, M(x_t))$, and $\alpha$ is the learning rate.

This novel perspective not only enriches the mathematical robustness of sequence-to-sequence learning problems but also makes provisions for incorporating clever optimization strategies endemic to reinforcement learning.

==> table/SLT_examples_full.tex <==
\begin{table*}
\centering
\setlength{\tabcolsep}{12pt}
\vspace{-0.3cm}
\begin{tabular}{lllcc}
\multicolumn{2}{l}{\small Example}   &                                                                                                                                                                                                                                                     & rBLEU & BLEU \\ 
\hline
\multicolumn{1}{|l}{\multirow{2}{*}{(1)}} & \multicolumn{1}{l}{Reference}  &  \begin{tabular}[c]{@{}l@{}}And that's a \textbf{great} \textbf{vital} \textbf{point} \textbf{technique} for \textbf{women's} \textbf{self} \textbf{defense}.\end{tabular}                                                                                                                                                                                                                                         & \multirow{2}{*}{30.29}                    & \multicolumn{1}{c|}{\multirow{2}{*}{38.25}} \\
\multicolumn{1}{|l}{}                     & \multicolumn{1}{l}{Prediction}  & It's really a \textbf{great} \textbf{point} for \textbf{women's} \textbf{self} \textbf{defense}.                                                                                                                                                                                                                                                                                                   &                                           & \multicolumn{1}{c|}{}                       \\ \hline
\multicolumn{1}{|l}{\multirow{2}{*}{(2)}} & \multicolumn{1}{l}{Reference}  & In this \textbf{clip} I'm going to \textbf{show} you how to \textbf{tape} your \textbf{cables} down.      & \multirow{2}{*}{24.88}   & \multicolumn{1}{c|}{\multirow{2}{*}{64.53}} \\
\multicolumn{1}{|l}{}                     & \multicolumn{1}{l}{Prediction}  & In this \textbf{clip} I'm going to \textbf{show} you how to \textbf{improve} \textbf{push} \textbf{ups}.                &                         & \multicolumn{1}{c|}{}    \\ \hline
\multicolumn{1}{|l}{\multirow{2}{*}{(3)}} & \multicolumn{1}{l}{Reference}  & \begin{tabular}[c]{@{}l@{}}In this \textbf{segment} we're going to \textbf{talk} about how to \textbf{load} your still for \\\textbf{distillation} of \textbf{lavender} \textbf{essential} \textbf{oil}.\\ -----\end{tabular}                                                                                                                                                                                               & \multirow{2}{*}{6.77}                     & \multicolumn{1}{c|}{\multirow{2}{*}{29.82}} \\
\multicolumn{1}{|l}{}                     & \multicolumn{1}{l}{Ours}  & \begin{tabular}[c]{@{}l@{}}\textbf{Ok}, in this \textbf{clip}, we're going to \textbf{talk} about how to \textbf{fold} the \textbf{ink} for \\ the \textbf{lid} of the \textbf{oil}.\end{tabular}                                                                                                                                                                                                                    &                                           & \multicolumn{1}{c|}{}                       \\ \hline
\multicolumn{1}{|l}{\multirow{2}{*}{(4)}} & \multicolumn{1}{l}{Reference}  & \begin{tabular}[c]{@{}l@{}}You are \textbf{dancing}, and now you are going to \textbf{need} the \textbf{veil} and you \\ are going to just \textbf{grab} the \textbf{veil} as \textbf{far} as \textbf{possible}.\\ -----\end{tabular}                                                                                                                                                                                        & \multicolumn{1}{c}{\multirow{2}{*}{4.93}} & \multicolumn{1}{c|}{\multirow{2}{*}{8.04}}  \\
\multicolumn{1}{|l}{}                     & \multicolumn{1}{l}{Ours.} & \begin{tabular}[c]{@{}l@{}}So, \textbf{once} you're \textbf{belly} \textbf{dancing}, \textbf{once} you've \textbf{got} to have the \textbf{strap}, \\ you're going to \textbf{need} to \textbf{grab} the \textbf{thumb}, and \textbf{try} to \textbf{avoid} it.\end{tabular}                                                                                                                                                                             & \multicolumn{1}{l}{}                      & \multicolumn{1}{l|}{}                       \\ \hline
\multicolumn{1}{|l}{\multirow{2}{*}{(5)}} & \multicolumn{1}{l}{Reference}  & \begin{tabular}[c]{@{}l@{}}But if you have to \textbf{setup} a \textbf{new campfire}, \textbf{there's two} \textbf{ways} to do \\ it in a very \textbf{low impact}; one is with a \textbf{mound fire}, which we should \\in the \textbf{campfire segment earlier} and the other way to \textbf{setup} a \textbf{low}\\ \textbf{impact campfire} is to have a \textbf{fire pan}, which is just a \textbf{steel pan} like \\ the \textbf{top} of a \textbf{trash} can.\\ -----\end{tabular} & \multirow{2}{*}{0.85}                     & \multicolumn{1}{c|}{\multirow{2}{*}{3.79}}  \\
\multicolumn{1}{|l}{}                     & \multicolumn{1}{l}{Ours}  & \begin{tabular}[c]{@{}l@{}}And other thing I'm going to \textbf{talk} to you is a little bit more \textbf{space}, \\ a \textbf{space} that's what it's going to do, it's \textbf{kind} of a \textbf{quick}, and then I \\don't want to take a \textbf{spray skirt} off, and then I don't want it to take\\ it to the \textbf{top} of it.\end{tabular}                                                              &                                           & \multicolumn{1}{c|}{}                       \\ \hline
\multicolumn{1}{|l}{\multirow{2}{*}{(6)}} & \multicolumn{1}{l}{Reference}  & \begin{tabular}[c]{@{}l@{}}So, this is a very \textbf{important} \textbf{part} of the \textbf{process}.\end{tabular}                                                                                  & \multirow{2}{*}{0.0}                        & \multicolumn{1}{c|}{\multirow{2}{*}{61.86}} \\
\multicolumn{1}{|l}{}                     & \multicolumn{1}{l}{Ours}  & It's a very \textbf{important} \textbf{part} of the \textbf{process}.                                                                                                                                                                                                                                                                                                            &                                           & \multicolumn{1}{c|}{}                       \\ \hline
\end{tabular}
\caption{Qualitative examples from our best-performing model. In bold the words remaining to compute rBLEU. Corresponding manually selected input frames from examples can be found in Appendix~\ref{appendix:examples_frames}}
\label{tab:SLT_examples}
\end{table*}

==> table/SLT_examples_short.tex <==
%\includegraphics[width=0.015\linewidth]{fig/y.drawio.png}

\begin{table*}[t]
\caption{\textbf{Concrete Cases Study:} We select some sample examples for readers to understand better. When using the prompt, we referred to the intermediate text, which would have made the measurement more accurate. Although there is still a problem that the accuracy is reduced due to the loss in the process of prompt-word to text. \textcolor{redongray}{Red} and \textcolor{blueongray}{Blue} mark similar part in the text in ASL and GSL, respectively.}
\label{tab:SLT_examples_short}
\centering
\setlength{\tabcolsep}{12pt}
%\vspace{-0.3cm}
\resizebox{1\linewidth}{!}{
%\begin{tabular}{lllcc}
%\includegraphics{table/slt.drawio.png}
%\end{tabular}
\begin{tabular}{lllll}
    \toprule
    \midrule
        Language & Format & Example & BLEU & ROUGE \\ \hline
        \multirow{2}{*}{(ASL)} & Reference (Text) &  \textcolor{redongray}{The} number one loss for these \textcolor{redongray}{birds}, is \textcolor{redongray}{flight}. & \multirow{2}{*}{20.21} & \multirow{2}{*}{62.86} \\ 
        ~ & Prediction & \textcolor{redongray}{The birds} couldn't lose the \textcolor{redongray}{flight}. & ~ & ~ \\ \hline
        \multirow{2}{*}{(GSL)} & Reference (Text) & Hoher \textcolor{blueongray}{luftdruck} sorgt bei uns morgen für viel \textcolor{blueongray}{sonnenschein}. & \multirow{2}{*}{10.1} & \multirow{2}{*}{56.43} \\ 
        ~ & Prediction & Morgen viel \textcolor{blueongray}{sonnenschein} wegen hohem \textcolor{blueongray}{luftdruck}. & ~ & ~ \\ \hline
        \multirow{3}{*}{(ASL)} & Prompt & What is the sign language for `When does this take place?'. & \multirow{3}{*}{40.00} & \multirow{3}{*}{40.00} \\ 
        ~ & Reference (LangGloss) & ASL\_\textcolor{redongray}{When} ASL\_\textcolor{redongray}{does} ASL\_this ASL\_take ASL\_place? & ~ & ~ \\ 
        ~ & Prediction & \textcolor{redongray}{When does} it takes up? & ~ & ~ \\ \hline
        \multirow{3}{*}{(GSL)} & Prompt & Wie gebärdet man `am freundlichsten wird es am meer' zeigen? & \multirow{3}{*}{57.14} & \multirow{3}{*}{73.4} \\ 
        ~ & Reference (LangGloss) & GSL\_\textcolor{blueongray}{Am} GSL\_\textcolor{blueongray}{freundlichsten} GSL\_\textcolor{blueongray}{wird} GSL\_\textcolor{blueongray}{es} GSL\_\textcolor{blueongray}{am} GSL\_meer. & ~ & ~ \\ 
        ~ & Prediction & \textcolor{blueongray}{Am} \textcolor{blueongray}{meer wird es am freundlichsten} sein. & ~ & ~ \\ 
        \midrule
        \bottomrule
    \end{tabular}
}
\vspace{-12pt}
\end{table*}

==> table/SM/3_code.tex <==
\begin{algorithm*}
  \SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
  \SetKwFunction{Union}{Union}\SetKwFunction{FindCompress}{FindCompress}
  \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}

  \Input{Three arrays $Xx$, $Xy$ and $Xw$ of size $T \times n$, a structure array, a sigma value for noise, a random number generator and a percentile value}
  \Output{Lines array, rootsx, rootsy, rootsz arrays, anglesx, anglesy, anglesz arrays, Yx, Yy, Yz arrays}
  \BlankLine
  \emph{Set T as number of rows and n as number of columns of $Xx$}\;
  
  \emph{Initialize arrays lines, rootsx, rootsy, rootsz, anglesx, anglesy, anglesz}\;
  
  \emph{Set rootsx as first column of $Xx$;Set rootsy as first column of $Xy$}\;
  \emph{Set rootsz as array of zeros with size T}\;
  
  \emph{Add noise to rootsx, rootsy, rootsz arrays}\;
  
  \emph{Initialize arrays Yx, Yy, Yz as arrays of zeros with size $T \times n$}\;
  \emph{Set first column of Yx as rootsx; Set first column of Yy as rootsy; Set first column of Yz as rootsz}\;
  
  \For{each bone in structure}{
    \emph{Add empty list to lines}\;
    \For{each row t in range T}{
      \emph{Compute length L using equation 1}\;
      \emph{Append L to lines}\;
    }
  }
  \For{each line in lines}{
    \emph{Calculate max L as percentile of the line list}\;
    \emph{Assign math.log(max L) to lines array}\;
  }
  
  \For{each bone in structure}{
    \emph{Assign a, b, line as elements of the bone}\;
    \For{each row t in range T}{
      \emph{Compute rotation angles anglex, angley, anglez using equation 2}\;
      \If{any of anglex, angley, anglez is not finite}{
        \emph{Set anglex, angley, anglez as 0.0}\;
      }
      \If{anglez < 0.0}{
        \emph{Set anglez as -anglez}\;
      }
      \emph{Add 0.001 to anglez}\;
      \emph{Normalize anglex, angley, anglez}\;
      \emph{Assign anglex, angley, anglez to anglesx[t, iBone], anglesy[t, iBone], anglesz[t, iBone]}\;
      \emph{Compute new 3D coordinates Yx, Yy, Yz using equation 3}\;
    }
  }
  
  \emph{Reshape rootsx, rootsy, rootsz as arrays of size T $\times$ 1}\;
  
  \emph{Return lines, rootsx, rootsy, rootsz, anglesx, anglesy, anglesz, Yx, Yy, Yz}\;

  %\vspace{12pt}
   \caption{The core formula and code of 2D to 3D conversion.}\label{3_code}
   %\vspace{-12pt}
\end{algorithm*}
%\vspace{-12pt}

==> table/SM/prompt.tex <==
\begin{table}[h]
\caption{\textbf{Prompt Ablation Study:} We added a row of comparative data to the table, $T$ represents a model that uses Text2LangGloss, but does not use Prompt as input this time.}
\label{tab:prompt_supp}
\centering
\resizebox{0.99\linewidth}{!}{%
\begin{tabular}{@{}p{3.0cm}ccccc@{}}
\toprule
     & \multicolumn{2}{c}{DEV SET}  & \multicolumn{2}{c}{TEST SET} \\
\multicolumn{1}{c}{Approach:}  & \multicolumn{1}{c}{BLEU-4 $\uparrow$} & \multicolumn{1}{c}{ROUGE $\uparrow$} & \multicolumn{1}{c}{BLEU-4 $\uparrow$} & \multicolumn{1}{c}{ROUGE $\uparrow$} \\ \midrule
\multicolumn{1}{r|}{Baseline \cite{stoll2018sign}} & 16.34 & 48.42 & 15.26 & 48.10 \\
\multicolumn{1}{r|}{Stoll et al. \cite{saunders2020progressive}} & 20.23 & 55.41 & 19.10 & 54.55 \\
\multicolumn{1}{r|}{\textbf{T (no prompt)}} & \textbf{22.45} & \textbf{53.56} & \textbf{20.12} & \textbf{51.37} \\
\multicolumn{1}{r|}{\textbf{Ours}} & \textbf{23.10} & \textbf{58.76} & \textbf{22.05} & \textbf{56.46} \\
\bottomrule
\end{tabular}%
}
% \vspace{}
\vspace{-14pt}
\end{table}

==> table/SM/prompt_temp_short.tex <==
% \begin{table*}[p]
%     \centering
%     \begin{tabularx}{\textwidth}{|X|}
%     \hline
%         \textbf{Prompt Template \& Some Examples} \hline
% & ~ \textbf{Part I}\\
% I really want to learn how to say ``\{\texttt{Text}\}'' in sign language. Can you help me?\\
% How would you express ``\{\texttt{Text}\}'' in sign language?\\
% Can you show me how to say ``\{\texttt{Text}\}'' in sign language?\\
% How do I say ``\{\texttt{Text}\}'' in sign language?\\ 
% Could you tell me how ``\{\texttt{Text}\}'' is represented in sign language?\\
% What is the sign language for ``\{\texttt{Text}\}''?& ~  \hline
% & ~ \textbf{Part II}\\
% How is ``So we're going to go up and down; let's switch hands, down and up; down and up.'' denoted in sign language?\\
% Can you elucidate how And just let those fingers relax. looks in sign language?\\
% I really want to learn how Now together you're going to go opposite. is said in sign language. Can you help?\\
% How do I articulate ``It's real easy to actually get your fingers to lead, so try not to let them do that.'' using sign language?\\
% I am intrigued to learn the sign language for `Let the wrist do all the leading.'.\\
% I am wondering how ``Don't let the fingers take over, let the wrist do all the guiding.'' appears in sign language. & ~  \hline
% & ~ \textbf{Part III}\\
% Ich möchte wirklich lernen wie man ``\{\texttt{Text}\}'' in Gebärdensprache sagt. Können Sie mir helfen?\\
% Wie würden Sie ``\{\texttt{Text}\}'' in Gebärdensprache ausdrücken?\\
% Können Sie mir zeigen wie man ``\{\texttt{Text}\}'' mit Gebärdensprache sagt?\\
% Wie sage ich ``\{\texttt{Text}\}'' in Gebärdensprache?\\
% Könnten Sie mir sagen wie ``\{\texttt{Text}\}'' in Gebärdensprache dargestellt wird?\\
% Was ist die Gebärdensprache für ``\{\texttt{Text}\}''? & ~  \hline
% & ~ \textbf{Part IV}\\
% 'regen und schnee lassen an den alpen in der nacht nach im norden und nordosten fallen hier und da schauer sonst ist das klar' Wie stellt man das in Gebärdensprache dar?\\
% %Können Sie die Gebärdensprache für 'am donnerstag regen in der nordhälfte in der südhälfte mal sonne mal wolken ähnliches wetter dann auch am freitag' demonstrieren?\\
% %Mich interessiert, wie vom nordmeer zieht ein kräftiges tief heran und bringt uns ab den morgenstunden heftige schneefälle zum teil auch gefrierenden regen in Gebärdensprache aussieht.\\
% Wie wird sonnig geht es auch ins wochenende samstag ein herrlicher tag mit temperaturen bis siebzehn grad hier im westen in Gebärdensprache dargestellt?\\
% Wie würden Sie deutschland liegt morgen unter hochdruckeinfluss der die wolken weitgehend vertreibt gebärden?\\
% Können Sie mir zeigen, wie am sonntag im nordwesten eine mischung aus sonne und wolken mit einigen zum teil gewittrigen schauern in Gebärdensprache aussieht?\\
% Wie sieht die Gebärdensprache für örtlich schauer oder gewitter die heftig sein können aus?\\
% Was ist die Gebärdensprache für und zum wochenende wird es dann sogar wieder ein bisschen kälter? & ~  \hline
%     \end{tabularx}
%     %\vspace{-4pt}
%     \caption{We provide two templates for sign language as a reference, and \texttt{\{Text\}} is where the video oral dialogue is inserted.}
%     %\vspace{-12pt}
%     \label{tab:temp_supp}
% \end{table*}

\begin{table*}[p]
    \centering
    \begin{tabularx}{\textwidth}{|X|} % Correct column specification
    \hline
    \textbf{Prompt Template \& Some Examples} \\ \hline
    \textbf{Part I} \\ \hline
    I really want to learn how to say ``\{\texttt{Text}\}'' in sign language. Can you help me? \\ \hline
    How would you express ``\{\texttt{Text}\}'' in sign language? \\ \hline
    Can you show me how to say ``\{\texttt{Text}\}'' in sign language? \\ \hline
    How do I say ``\{\texttt{Text}\}'' in sign language? \\ \hline
    Could you tell me how ``\{\texttt{Text}\}'' is represented in sign language? \\ \hline
    What is the sign language for ``\{\texttt{Text}\}''? \\ \hline
    \textbf{Part II} \\ \hline
    How is ``So we're going to go up and down; let's switch hands, down and up; down and up.'' denoted in sign language? \\ \hline
    Can you elucidate how ``And just let those fingers relax.'' looks in sign language? \\ \hline
    I really want to learn how ``Now together you're going to go opposite.'' is said in sign language. Can you help? \\ \hline
    How do I articulate ``It's real easy to actually get your fingers to lead, so try not to let them do that.'' using sign language? \\ \hline
    I am intrigued to learn the sign language for ``Let the wrist do all the leading.'' \\ \hline
    I am wondering how ``Don't let the fingers take over, let the wrist do all the guiding.'' appears in sign language. \\ \hline
    \textbf{Part III} \\ \hline
    Ich möchte wirklich lernen wie man ``\{\texttt{Text}\}'' in Gebärdensprache sagt. Können Sie mir helfen? \\ \hline
    Wie würden Sie ``\{\texttt{Text}\}'' in Gebärdensprache ausdrücken? \\ \hline
    Können Sie mir zeigen wie man ``\{\texttt{Text}\}'' mit Gebärdensprache sagt? \\ \hline
    Wie sage ich ``\{\texttt{Text}\}'' in Gebärdensprache? \\ \hline
    Könnten Sie mir sagen wie ``\{\texttt{Text}\}'' in Gebärdensprache dargestellt wird? \\ \hline
    Was ist die Gebärdensprache für ``\{\texttt{Text}\}''? \\ \hline
    \textbf{Part IV} \\ \hline
    'Regen und Schnee lassen an den Alpen in der Nacht nach, im Norden und Nordosten fallen hier und da Schauer, sonst ist das klar' Wie stellt man das in Gebärdensprache dar? \\ \hline
    %Können Sie die Gebärdensprache für 'am Donnerstag Regen in der Nordhälfte, in der Südhälfte mal Sonne mal Wolken, ähnliches Wetter dann auch am Freitag' demonstrieren? \\ \hline
    %Mich interessiert, wie 'vom Nordmeer zieht ein kräftiges Tief heran und bringt uns ab den Morgenstunden heftige Schneefälle, zum Teil auch gefrierenden Regen' in Gebärdensprache aussieht. \\ \hline
    Wie wird 'Sonnig geht es auch ins Wochenende, Samstag ein herrlicher Tag mit Temperaturen bis siebzehn Grad hier im Westen' in Gebärdensprache dargestellt? \\ \hline
    Wie würden Sie 'Deutschland liegt morgen unter Hochdruckeinfluss, der die Wolken weitgehend vertreibt' gebärden? \\ \hline
    Können Sie mir zeigen, wie 'am Sonntag im Nordwesten eine Mischung aus Sonne und Wolken mit einigen zum Teil gewittrigen Schauern' in Gebärdensprache aussieht? \\ \hline
    Wie sieht die Gebärdensprache für 'örtlich Schauer oder Gewitter, die heftig sein können' aus? \\ \hline
    Was ist die Gebärdensprache für 'und zum Wochenende wird es dann sogar wieder ein bisschen kälter'? \\ \hline
    \end{tabularx}
    %\vspace{-4pt}
    \caption{We provide two templates for sign language as a reference, and \texttt{\{Text\}} is where the video oral dialogue is inserted.}
    %\vspace{-12pt}
    \label{tab:temp_supp}
\end{table*}


==> table/ablation.tex <==
\begin{table*}[ht]
\caption{\textbf{Comparison of Different Modules:} \ourLLMmethodName{}-40M-Base results for \textit{Text to Pose} task on the ASL part of \ourDataName{}, with multiple data augmentation techniques. Base: Multi-Language Switching Framework with Normal MSE Loss, no enhancement Settings. FP: Future Prediction. GN: Gaussian Noise. Prompt2LangGloss: Prompt2LangGloss with Normal MSE Loss. PLC: Priority Learning Channel. The \textcolor{sgreen}{\small{\textbf{increase number}}} is compared to the base model. The \textcolor{blueongray}{blue areas} are our results, the \textcolor{gray}{gray areas} are for reference, and the other lines are traditional techniques. Top performances are highlighted in \textbf{bold}, while second top performances are \underline{underlined}.}
%\vspace{-0.3cm}
\label{tab:data_augmentation_results}
\centering
\resizebox{1\linewidth}{!}{%
\begin{tabular}{@{}p{2.8cm}ccccc|ccccc@{}}
\toprule
\midrule
     & \multicolumn{5}{c}{DEV SET}  & \multicolumn{5}{c}{TEST SET} \\ 
\multicolumn{1}{c|}{Approach:}  & BLEU-4         & BLEU-3         & BLEU-2         & BLEU-1         & ROUGE          & BLEU-4         & BLEU-3         & BLEU-2         & BLEU-1         & ROUGE          \\ \midrule
\rowcolor{backgroundgray} \multicolumn{1}{r|}{\textbf{\color{gray} Base}} & \color{gray} 10.96 & \color{gray} 14.68 & \color{gray} 22.49 & \color{gray} 40.29 & \color{gray} 44.13 & \color{gray} 9.27 & \color{gray} 10.72 & \color{gray} 18.64 & \color{gray} 39.88 & \color{gray} 40.39 \\
\multicolumn{1}{r|}{Future Prediction} & 13.48 & 18.64 & 27.69 & 46.88 & 48.45 & 13.76 & 16.21 & 25.88 & 44.57 & 46.47 \\
\multicolumn{1}{r|}{Just Counter} & 15.29 & 21.98 & 29.72 & 48.54 & 50.95 & 13.73 & 17.02 & 27.65 & 47.71 & 48.79 \\
\multicolumn{1}{r|}{Gaussian Noise} & 16.28 & 23.53 & 32.05 & 50.76 & 53.68 & 15.63 & 20.35 & 29.19 & 47.91 & 50.16 \\
\multicolumn{1}{r|}{FP \& GN} & 16.44 & 23.79 & 32.32 & 50.97 & 53.44 & \textbf{17.17} & \textbf{21.25} & \textbf{30.12} & \textbf{50.25} & 50.47 \\
\rowcolor{backgroundblue} \multicolumn{1}{r|}{\textbf{Prompt2LangGloss}}& 15.78 & 22.66 & 30.27 & 48.30 & 50.88 & \quad \underline{16.32}\textcolor{sgreen}{\small{\textbf{ +7.05}}} & \underline{20.27} & \underline{28.70} & \underline{47.89} & 48.18\\     
\rowcolor{backgroundblue} \multicolumn{1}{r|}{\textbf{RL Loss}}    & 18.33 & 24.28 & 32.18 & 48.83 & 52.61 & 13.26 & 17.33 & 24.51 & 40.76 & 40.95 \\ 
\rowcolor{backgroundblue} \multicolumn{1}{r|}{\textbf{RL Loss \& PLC}}       & \textbf{\quad 18.77}\textcolor{sgreen}{\small{\textbf{ +7.81}}} & \textbf{25.42} & \textbf{32.44} & \textbf{52.66} & \textbf{61.44} & 14.13 & 19.08 & 25.72 & 43.40 & \textbf{51.57} \\
\midrule
\bottomrule
\end{tabular}%
}
%\vspace{-4pt}
\vspace{-12pt}
\end{table*}

==> table/ablation_short_green.tex <==
\begin{table*}[ht]
%\vspace{-0.3cm}
\centering
\resizebox{1\linewidth}{!}{%
\begin{tabular}{@{}p{2.8cm}ccccc|ccccc@{}}
\toprule
\midrule
     & \multicolumn{5}{c}{DEV SET}  & \multicolumn{5}{c}{TEST SET} \\ 
\multicolumn{1}{c|}{Approach:}  & BLEU-4         & BLEU-3         & BLEU-2         & BLEU-1         & ROUGE          & BLEU-4         & BLEU-3         & BLEU-2         & BLEU-1         & ROUGE          \\ \midrule
%\rowcolor{backgroundgray} 
\multicolumn{1}{r|}{\textbf{\color{cancelgray} Base}} & \color{cancelgray} 10.96 & \color{cancelgray} 14.68 & \color{cancelgray} 22.49 & \color{cancelgray} 40.29 & \color{cancelgray} 44.13 & \color{cancelgray} 9.27 & \color{cancelgray} 10.72 & \color{cancelgray} 18.64 & \color{cancelgray} 39.88 & \color{cancelgray} 40.39 \\
%\rowcolor{backgroundblue} 
\multicolumn{1}{r|}{\textbf{Prompt2LangGloss}}& 15.78 & 22.66 & 30.27 & 48.30 & 50.88 & \quad \underline{16.32}\textcolor{sgreen}{\small{\textbf{ +7.05}}} & \underline{20.27} & \underline{28.70} & \underline{47.89} & 48.18\\     
%\rowcolor{backgroundblue} 
\multicolumn{1}{r|}{\textbf{RL Loss}}    & 18.33 & 24.28 & 32.18 & 48.83 & 52.61 & 13.26 & 17.33 & 24.51 & 40.76 & 40.95 \\ 
%\rowcolor{backgroundblue} 
\multicolumn{1}{r|}{\textbf{RL Loss \& PLC}}       & \textbf{\quad 18.77}\textcolor{sgreen}{\small{\textbf{ +7.81}}} & \textbf{25.42} & \textbf{32.44} & \textbf{52.66} & \textbf{61.44} & 14.13 & 19.08 & 25.72 & 43.40 & \textbf{51.57} \\
\midrule
\bottomrule
\end{tabular}%
}
\vspace{-6pt}
\caption{\textbf{Comparison of Different Modules:} \ourLLMmethodName{}-40M-Base results for \textit{Text to Pose} task on the ASL part of \ourDataName{}, with multiple data augmentation techniques. Base: Multi-Language Switching Framework with Normal MSE Loss, no enhancement Settings. Prompt2LangGloss: Prompt2LangGloss with Normal MSE Loss. PLC: Priority Learning Channel. The \textcolor{sgreen}{\small{\textbf{increase number}}} is compared to the base model. 
%The \textcolor{blueongray}{blue areas} are our results, the \textcolor{gray}{gray areas} are for reference, and the other lines are traditional techniques. 
Top performances are highlighted in \textbf{bold}, while second top performances are \underline{underlined}.}\label{tab:data_augmentation_results}
%\vspace{-4pt}
\vspace{-12pt}
\end{table*}

==> table/aslp.tex <==
\begin{table*}[t]
%\vspace{-0.3cm}
\centering
\resizebox{1\linewidth}{!}{%
\begin{tabular}{@{}p{2.8cm}ccccc|ccccc@{}}
\toprule
\midrule
 & \multicolumn{5}{c}{DEV SET} & \multicolumn{5}{c}{TEST SET} \\ 
\multicolumn{1}{c|}{Type:} & BLEU-4         & BLEU-3         & BLEU-2         & BLEU-1         & ROUGE          & BLEU-4         & BLEU-3         & BLEU-2         & BLEU-1         & ROUGE          \\ \midrule
%\multicolumn{1}{r|}{Saunders \etal \cite{saunders2020progressive}}     &  11.82 &  14.80 & 19.97 & 31.41 & 33.18 & 10.51 & 13.54 & 19.04 & 31.36 & 32.46 \\
\multicolumn{1}{r|}{NSLP-G \cite{hwang2021non}}   & - & - & - & - & - & 5.75 & 8.21 & 11.62 & 17.55 & 31.98 \\
\multicolumn{1}{r|}{Fast-SLP Transformers \cite{fang2024signdiffdiffusionmodelsamerican}}  & 17.19 & 23.11 & 29.49 & 36.96 & 55.85 & 12.85 & 17.35 & 23.38 & 39.46 & 46.89 \\
%\midrule
\multicolumn{1}{r|}{Neural Sign Actors \cite{Baltatzis_2024_CVPR}}   & - & - & - & - & - & 13.12 & 18.25 & 25.44 & 41.31 & 47.55 \\
\midrule
%\rowcolor{backgroundblue} 
\multicolumn{1}{r|}{\textbf{SignLLM-1x40M-Base-M (ASL) }}   & 18.77 & 25.42 & 32.44 & 40.66 & 61.44 & 14.13 & 19.08 & 25.72 & 43.40 & 51.57 \\
%\rowcolor{backgroundblue} 
\multicolumn{1}{r|}{\textbf{SignLLM-1x120M-Large-M (ASL) }}   & 19.40 & 26.11 & 33.38 & 41.89 & 63.21 & 14.52 & 19.65 & 26.44 & 44.72 & 53.14 \\
%\rowcolor{backgroundblue} 
\multicolumn{1}{r|}{\textbf{SignLLM-1x1B-Super-M (ASL) }}   & \textbf{\quad 20.09}\textcolor{sgreen}{\small{\textbf{ +2.9}}} & \textbf{27.04} & \textbf{34.45} & \textbf{43.16} & \textbf{65.19} & \textbf{\quad 15.03}\textcolor{sgreen}{\small{\textbf{ +2.18}}} & \textbf{20.28} & \textbf{27.35} & \textbf{46.17} & \textbf{54.86} \\
\midrule
%\rowcolor{backgroundgray} 
\multicolumn{1}{r|}{\textbf{\color{cancelgray} SignLLM-1x40M-Base-P (ASL) }}   & \color{cancelgray} 17.34 & \color{cancelgray} 23.57 & \color{cancelgray} 29.87 & \color{cancelgray} 37.81 & \color{cancelgray} 56.93 & \color{cancelgray} 13.06 & \color{cancelgray} 17.66 & \color{cancelgray} 23.77 & \color{cancelgray} 40.15 & \color{cancelgray} 47.76 \\
%\rowcolor{backgroundgray} 
\multicolumn{1}{r|}{\textbf{\color{cancelgray} SignLLM-1x120M-Large-P (ASL) }}   & \color{cancelgray} 18.05 & \color{cancelgray} 24.28 & \color{cancelgray} 31.04 & \color{cancelgray} 38.97 & \color{cancelgray} 58.78 & \color{cancelgray} 13.48 & \color{cancelgray} 18.27 & \color{cancelgray} 24.57 & \color{cancelgray} 41.57 & \color{cancelgray} 49.42 \\
%\rowcolor{backgroundgray} 
\multicolumn{1}{r|}{\textbf{\color{cancelgray} SignLLM-1x1B-Super-P (ASL) }}   & \color{cancelgray} \textbf{\quad 18.68}\textcolor{sgreen}{\small{\textbf{ +1.49}}} & \color{cancelgray} 25.11 & \color{cancelgray} 31.99 & \color{cancelgray} 40.14 & \color{cancelgray} 60.47 & \color{cancelgray} \textbf{\quad 13.93}\textcolor{sgreen}{\small{\textbf{ +0.92}}} & \color{cancelgray} 18.86 & \color{cancelgray} 25.40 & \color{cancelgray} 42.87 & \color{cancelgray} 50.91 \\
\midrule
\bottomrule
\end{tabular}%
}
\vspace{-6pt}
\caption{
\textbf{\acf{aslp}:} Comparison of \ourLLMmethodName{} variants with baseline on \textit{Text to Pose} task by using our \ourDataName{} ASL part. The \textcolor{sgreen}{\small{\textbf{increase number}}} is compared to one of the latest work \cite{fang2024signdiffdiffusionmodelsamerican,Baltatzis_2024_CVPR}.
%The \textcolor{blueongray}{blue areas} and the \textcolor{gray}{gray areas} stand for the result of two modes.
%Models $M$ and $P$ represent MLSF and Prompt2LangGloss trained ASLP models, respectively.
}\label{tab:aslp}
%\vspace{-6pt}
\vspace{-12pt}
\end{table*}

==> table/datasets_all.tex <==
\begin{table*}[t]
\caption{\textbf{Comparison of Dataset Details:}
\ourDataName{} uses tools to automate the acquisition and processing of sign language videos on the web, is a better dataset that is efficient (a higher level of preprocessing, standardized and more models available), and lightweight (average reduction of 80\% in space usage).
%, reducing the previous shortcomings both in terms of the tools and the data itself. 
%Languages 
Included: American Sign Language (ASL), German Sign Language (GSL, Alias DGS), Swiss German Sign Language (DSGS), French Sign Language of Switzerland (LSF-CH), Italian Sign Language of Switzerland (LIS-CH), Argentine Sign Language (Lengua de Señas Argentina, LSA), Korean Sign Language (KSL), and Turkish Sign Language (TSL).
%Languages such as Chinese Sign Language and Spanish Sign Language will also be included in the future.
}
%\vspace{-13pt}
\vspace{-5pt}
\label{tab:related_datasets_all}
\centering
\renewcommand{\arraystretch}{1.2}
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccccccc} 
    \hline
    \midrule
        \textbf{Name}                            & \textbf{Language} & \textbf{Vocab.} & \textbf{Duration (h)} & \textbf{Signers} & \textbf{Multiview} & \textbf{Transcription} & \textbf{Gloss} & \textbf{Pose} & \textbf{Depth} & \textbf{Speech} & \textbf{Prompt} & \textbf{Compress}\\
    \hline                          
        Video-Based CSL~\cite{video-based}       & CSL               & 178       & 100           & 50 &\xmark & \greencheck & \xmark     & \greencheck     & \greencheck   & \xmark  & \xmark & \xmark\\
        SIGNUM~\cite{SIGNUM}                     & GSL               & 450       & 55            & 25 &\xmark     & \greencheck & \greencheck & \xmark     & \xmark   & \xmark & \xmark & \xmark \\
        RWTH-Phoenix-2014T~\cite{SLTranslation}  & GSL               & 3k        & 11            & 9 &\xmark     & \greencheck & \greencheck & \xmark     & \xmark   & \xmark & \xmark & \xmark \\
        Public DGS Corpus~\cite{DGS-Korpus}      & GSL               & --        & 50            & 327 &\greencheck & \greencheck & \greencheck & \greencheck & \xmark   & \xmark & \xmark & \xmark \\
        %BSL1k~\cite{BSL-1K}                      & BSL               & 1k        & 1000          & \xmark     & \greencheck & \greencheck & \xmark     & \xmark   & \xmark \\ 
        BSL Corpus~\cite{bsl-corpus}             & BSL               & 5k        & --            & 249 &\xmark     & \greencheck & \greencheck & \xmark     & \xmark   & \xmark & \xmark & \xmark \\ 
    \hline
        NCSLGR~\cite{NCSLGR}                     & ASL               & 1.8k     & 5.3            & 4 &\greencheck & \greencheck & \greencheck & \xmark     & \xmark     & \xmark & \xmark & \xmark \\
        How2Sign \cite{duarte2021how2sign}                 & ASL               & 16k       & 79            & 11 &\greencheck & \greencheck & \greencheck & \greencheck & \greencheck & \greencheck & \xmark & \xmark \\
    \hline
       \rowcolor{backgroundblue} \textbf{Prompt2Sign (ours)}                 & Multilingual               & 40k       & 200            & 40 &\greencheck & \greencheck & \greencheck & \greencheck & \greencheck & \greencheck & \greencheck & \greencheck \\
    \hline
    \midrule
\end{tabular}
}
%\vspace{-5pt}
\vspace{-8pt}
\end{table*}
\vspace{-12pt}
%\noindent \textsuperscript{*}{\tiny Languages included: American Sign Language (ASL), German Sign Language (GSL, Alias DGS), Swiss German Sign Language (DSGS), French Sign Language of Switzerland (LSF-CH), Italian Sign Language of Switzerland (LIS-CH), Argentine Sign Language (Lengua de Señas Argentina, LSA), Korean Sign Language (KSL), and Turkish Sign Language (TSL).}
%\tablefootnote{Languages included: American Sign Language (ASL), German Sign Language (GSL, Alias DGS), Swiss German Sign Language (DSGS), French Sign Language of Switzerland (LSF-CH), Italian Sign Language of Switzerland (LIS-CH), Argentine Sign Language (Lengua de Señas Argentina, LSA), Korean Sign Language (KSL), and Turkish Sign Language (TSL).}
%\footnotesize{$^a$ The smallest spatial unit is county, $^b$ more details in appendix A}
%\footnotetext{The specific data may vary, so please refer to the actual information for accuracy.}

==> table/datasets_overview.tex <==
\begin{table}[t]
\begin{minipage}{0.48\linewidth}
  \centering
  \includegraphics[width=\textwidth]{fig/ratar.png}
  \label{fig:a}
  \vspace{-12pt}
\end{minipage}\hspace*{0.04\linewidth}%\hfill
\begin{minipage}{0.48\linewidth}
  \centering
  \includegraphics[width=\textwidth]{fig/data_map.png}
  \label{fig:b}
  \vspace{-12pt}
\end{minipage}
    \\
    \vspace{4pt} \makebox[0.222\textwidth][c]{(a)} \makebox[0.24\textwidth][c]{\hspace{1em}(b)} \vspace{-10pt}
    \caption{\textbf{Our comparison with other mainstream datasets \cite{koller15:cslr, Duarte_2021_how2sign, video-based}:}
(a) represents whether the three data sets have a certain property, for example, the \textcolor[rgb]{1,0.749,1}{Phoenix-2014T} just has Gloss and Transcription, the \textcolor[rgb]{0.749,0.749,1}{Video-Based CSL} just has Pose and Depth, so their area are the smallest. (b) represents the number of video clips in their \textcolor[rgb]{0.713,0.188,0.110}{train}, \textcolor[rgb]{1,0.871,0.255}{dev}, \textcolor[rgb]{0,0.686,0.702}{test} set, respectively. 
%More information can be found in the supplementary material.
}
\vspace{-13pt}
\label{tab:related_datasets_radar}
\end{table}
%(b) represents the number of video clips in their \textcolor[rgb]{0.756,0.121,0.121}{training} \textcolor[rgb]{1,0.576,0.098}{development} \textcolor[rgb]{1,0.792,0.105}{test} set. More information can be found in the supplementary material.}

==> table/datasets_short.tex <==
\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.2}
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccccc} 
    \hline
    \midrule
        \textbf{Name}                            & \textbf{Language} & \textbf{Vocab.} & \textbf{Duration (h)}  &  \multicolumn{7}{c}{\textbf{Modalities}} \\
                                                 &                   &           &               & &\textbf{Multiview}  & \textbf{Gloss} & \textbf{Pose} & \textbf{Depth} & \textbf{Speech} & \textbf{Prompt} & \textbf{Compress}\\
    \hline                          
        Video-Based CSL~\cite{video-based}       & CSL               & 178       & 100            &\xmark  & \xmark     & \bluecheck     & \bluecheck   & \xmark  & \xmark & \xmark\\
        SIGNUM~\cite{SIGNUM}                     & GSL               & 450       & 55             &\xmark      & \bluecheck & \xmark     & \xmark   & \xmark & \xmark & \xmark \\
        RWTH-Phoenix-2014T~\cite{SLTranslation}  & GSL               & 3k        & 11             &\xmark     & \bluecheck & \xmark     & \xmark   & \xmark & \xmark & \xmark \\
        Public DGS Corpus~\cite{DGS-Korpus}      & GSL               & --        & 50             &\bluecheck  & \bluecheck & \bluecheck & \xmark   & \xmark & \xmark & \xmark \\
        %BSL1k~\cite{BSL-1K}                      & BSL               & 1k        & 1000          & \xmark     & \bluecheck & \bluecheck & \xmark     & \xmark   & \xmark \\ 
        BSL Corpus~\cite{bsl-corpus}             & BSL               & 5k        & --             &\xmark     & \bluecheck & \xmark     & \xmark   & \xmark & \xmark & \xmark \\ 
    \hline
        NCSLGR~\cite{NCSLGR}                     & ASL               & 1.8k     & 5.3             &\bluecheck  & \bluecheck & \xmark     & \xmark     & \xmark & \xmark & \xmark \\
        How2Sign \cite{duarte2021how2sign}                 & ASL               & 16k       & 79             &\bluecheck  & \bluecheck & \bluecheck & \bluecheck & \bluecheck & \xmark & \xmark \\
    \hline
        \textbf{Prompt2Sign (ours)}                 & ASL\&GSL               & 21k       & 90            &\bluecheck  & \bluecheck & \bluecheck & \bluecheck & \bluecheck & \bluecheck & \bluecheck \\
    \hline
    \midrule
\end{tabular}
}
\vspace{-5pt}
\caption{\textbf{Summary of previous mainstream sign language datasets:}
Our \ourDataName{}, which uses tools to automate the acquisition and processing of sign language videos on the web, is an evolving data set that is efficient and lightweight without the previous shortcomings. Languages such as Chinese Sign Language and British Sign Language will also be included in the future.
}
\vspace{-13pt}
\label{tab:related_datasets_short}
\end{table}

==> table/datasets_slt.tex <==
\begin{table*}[!ht]
\caption{Comparison between SLT datasets based on the duration of the videos (in hours), number of unique words (in thousands) in the vocabulary and SOTA on SLT without glosses. $\leftarrow$ $\rightarrow$ indicate that in some cases only statistics on the whole dataset are provided.}
\label{tab:SLT_datasets}
\centering
\begin{tabular}{lcccccccl}
\toprule
Dataset                                                                               & \multicolumn{3}{c}{Duration(h)} & \multicolumn{3}{c}{Vocabulary(K)}                                              & BLEU                                                                   & Domain                 \\
 & train     & val      & test     & \multicolumn{1}{l}{train} & \multicolumn{1}{l}{val} & \multicolumn{1}{l}{test} &                                                                                  &                        \\ \midrule
KETI~\cite{Ko-2019-SLT-based-human-keypoint-estimation}                              & 20.05     & 2.24     & 5.70     & $\leftarrow$ & 0.49 & $\rightarrow$                                                       & 57.37~\cite{Ko-2019-SLT-based-human-keypoint-estimation}   & Emergency situations   \\
PHOENIX-2014T~\cite{2018_Neural_Sign_Language_Translation}                           & 9.2       & 0.6      & 0.7      & 2                         & 0.9                     & 1                        & 25.59~\cite{Vskou-2021-stochastic-transformer-SLT}   & Weather Forecast       \\
CSL Daily~\cite{Zhou2021ImprovingSLT-with-monolingual-CSLDaily}                      & 20.62     & 1.24     & 1.41     & 2                         & 1.3                     & 1.3                      & 23.92~\cite{chen2022simple} & Daily life             \\
OpenASL~\cite{shi-etal-2022-openASL}                            & $\leftarrow$ & 288  & $\rightarrow$          & $\leftarrow$ & 33 &$\rightarrow$                                                         & 6.72~\cite{shi-etal-2022-openASL}                          & Youtube (news + vlogs) \\ \midrule
How2Sign~\cite{Duarte_2021_how2sign}                          & 69.6      & 3.9      & 5.6      & 15.6                      & 3.2                     & 3.6                      & 8.03 (Ours)                                                                      & Instructional          \\ \bottomrule
\end{tabular}
\vspace{-12pt}
\end{table*}

==> table/namingrule.tex <==
%\begin{wraptable}{r}{6.5cm}
\begin{table*}[ht]
%\vspace{-0.50cm}
\centering
\caption{\textbf{Naming Rule:} $M$ and $P$ represent MLSF and Prompt2LangGloss, respectively. Adress represents which traditional step has been innovated, while Features represents the ability of the mode to focus more on.}
\label{tab:naming}
\vspace{-6pt}
\resizebox{1\textwidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|}
    \hline
        SignLLM & \{number of language\}x & \{single language parameters\} & \{submode size\} & \{the mode of training\} & \{the language of input\} \\ \hline
        模型名称 & \{1，2，3...\} & \{20，40，etc\} & \{Base, Large, Super\} & \{M (MLSF), P (Prompt2LangGloss)\} & \{ASL, GSL, etc\} \\ \hline
\end{tabular}
}
\vspace{-1pt}
\end{table*}
%\vspace{-0.65cm}
%\end{wraptable}

==> table/visual.tex <==
\begin{table}[t!]
\centering
\resizebox{0.99\linewidth}{!}{%
\begin{tabular}{@{}p{3.0cm}ccccc@{}}
\toprule
  & \multicolumn{1}{c}{SSIM $\uparrow$} & \multicolumn{1}{c}{Hand SSIM $\uparrow$} & \multicolumn{1}{c}{Similarity $\uparrow$} & \multicolumn{1}{c}{F2FD $\downarrow$} \\ \midrule
\multicolumn{1}{r|}{Vid2Vid \cite{wang2018video}} & 0.743 & 0.582 & 78.42 & 27.86 \\
\multicolumn{1}{r|}{ControlNet \cite{zhang2023adding}} & 0.817 & 0.646 & 82.11 & 25.47 \\
\multicolumn{1}{r|}{Motion Capture} & \textbf{0.826} & \textbf{0.687} & \textbf{81.29} & \textbf{22.71} \\
\bottomrule
\end{tabular}%
}
\vspace{-1mm}
\caption{\textbf{Visual Study:} SSIM: Comparison of image structure similarity between the generated image and the condition graph extracted from the Ground Truth. Similarity: Extract the similarity percentage of keypoints between the generated video and the input action. F2FD: The degree of difference between frames.}
\label{tab:visual}
% \vspace{}
\vspace{-12pt}
\end{table}
